Mirror Sinkhorn: Fast Online Optimization on Transport Polytopes

Optimal transport is an important tool in machine learning, allowing to capture geometric properties of the data through a linear program on transport polytopes. We present a single-loop optimization algorithm for minimizing general convex objectives on these domains, utilizing the principles of Sinkhorn matrix scaling and mirror descent. The proposed algorithm is robust to noise, and can be used in an online setting. We provide theoretical guarantees for convex objectives and experimental results showcasing it effectiveness on both synthetic and real-world data.

==> preamble.tex <==
% If accepted, instead use the following line for the camera-ready submission:
% \usepackage[accepted]{icml2023}

% For theorems and such
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

% if you use cleveref..
\usepackage[capitalize,noabbrev]{cleveref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

%%%%%%%%%%%%%%%% Commandes %%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\Hull}{Hull}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\KL}{KL}
\DeclareMathOperator{\Diag}{Diag}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\ROUND}{\mathcal{R}}
\newcommand{\radius}{\delta}
\newcommand{\Esp}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\ndqb}[1]{\textcolor{red}{\textbf{[QB: #1]}}}
\newcommand{\ndmb}[1]{\textcolor{blue}{\textbf{[MB: #1]}}}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{xcolor}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{booktabs}
% for professional tables
\usepackage[algo2e]{algorithm2e} 
\usepackage{float}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{bbm}
\usepackage{float}
\usepackage[colorlinks=true,citecolor=blue,allcolors=blue]{hyperref}
\usepackage{etoolbox}
\usepackage{breakcites}

\newcommand{\isarxiv}{0}

==> sections/0--title_arxiv.tex <==
\title{Mirror Sinkhorn: Fast Online\\ Optimization on Transport Polytopes}
\author{	Marin Ballu\thanks{
  Department of Pure Mathematics and Mathematical Statistics, University of Cambridge,
	\texttt{mb2193@cam.ac.uk} }
	\and
  Quentin Berthet\thanks{
  Google Research, Brain team, Paris,
  \texttt{qberthet@google.com}
  }
}
\maketitle


==> sections/6-acks.tex <==
\section*{Acknowledgements} Marin Ballu is supported by the Cantab Capital Institute for Mathematics of Information. The authors would like to thank Jonathan Niles-Weed for discussions on this problem, and Laetitia~Meng-Papaxanthos for pointing them towards the SNARE-seq data. 

==> sections/theorems/alg_var.tex <==
\begin{algorithm}[hbt!]
\caption{Mirror Monge (var)}\label{alg:var}
\KwData{Initialise $\gamma_1 =\overline{\gamma}_1= \mu\nu^\top$, stepsize parameter $\eta>0$.}
\For{$1\leq t\leq T$}{
Compute error $c_t = \Vert\gamma_t1_n-\mu\Vert_1 + \Vert(\gamma_t)^\top1_m-\nu\Vert_1$,\\
Compute stepsize $\eta_t = \eta c_t$,\\
Update $\gamma_{t+1}' = \gamma_{t} \odot \exp\left(- \eta_t \nabla f(\gamma_t)\right),$\\
\eIf{$t$ is even}{
Normalise rows $\gamma_{t+1} = \Diag\left(\frac{\mu}{\gamma_{t+1}'1_n}\right)\gamma_{t+1}'$,
}{
Normalise columns $\gamma_{t+1} = \gamma_{t+1}'\Diag\left(\frac{\nu}{(\gamma_{t+1}')^\top1_m}\right)$,
}
Update $\overline{\gamma}_{t+1} = \frac{t}{t+1}\overline{\gamma}_t + \frac{1}{t+1}\gamma_{t+1}$
}
\KwOut{$\overline{\gamma}_T = \frac{1}{T}\sum_{t=1}^T\gamma_t$ }

\end{algorithm}

==> sections/theorems/thm_smooth.tex <==
%\begin{thm}\label{thm:smooth}
We assume that $f$ is $L-$smooth for the norm $\Vert \cdot\Vert_1$, i.e.
\begin{equation}
    \langle\nabla f(\gamma) - \nabla f(\gamma'),\gamma - \gamma'\rangle\leq L\Vert\gamma'- \gamma\Vert_1^2
\end{equation}
for all probability matrices $\gamma, \gamma'\in\R_+^{m\times n}$.
let $0\leq\alpha<1$, let $B = \Vert\nabla f(\gamma^*)\Vert_\infty$, let the stepsize be $\eta_t = \frac{2}{L+2B}\sqrt{\frac{\radius}{t}}$ in the algorithm \ref{alg:main}, then the output $\overline{\gamma}_T$ after $T$ steps verifies
\begin{equation}
    f(\overline{\gamma}_T) - f(\gamma^*) \leq  \left(B+\frac{L}{2}\right) \sqrt{\frac{\radius}{T}}(2+\log(T)).
\end{equation}
and the constraints are close to be verified
\begin{equation}
    c(\overline{\gamma}_T)\leq 
\end{equation}
%\end{thm}

==> sections/theorems/thm_stoch.tex <==
%\begin{thm}\label{thm:stoch}
If $f$ is $B$-Lipschitz for the norm $\Vert\cdot\Vert_1$, and if
\begin{equation}
    \Esp{}{\Vert g_t - \nabla f(\gamma_t)\Vert_\infty^2\vert \gamma_t}\leq \sigma^2.
\end{equation}
Let $B_\sigma = \sqrt{B^2 +\sigma^2}$,
let the stepsize be $\eta_t = \frac{1}{B_\sigma}\sqrt{\frac{\radius}{t}}$  in the algorithm \ref{alg:stoch}, then the output $\overline{\gamma}_T$ after $T$ steps verifies
 \begin{equation}
    \Esp{}{f(\overline{\gamma}_T) - f(\gamma^*)} \leq  \frac{9B_\sigma}{8}\sqrt{\frac{\radius}{T}}(2+\log(T)),
\end{equation}
and the constraints are close to be verified
\begin{equation}
    \Esp{}{c(\overline{\gamma}_T)} \leq  \frac{3}{2}\sqrt{\frac{\radius}{T}}(2+\log(T)),
\end{equation}
with
\begin{equation}
    c(\overline{\gamma}_T) = \Vert\overline{\gamma}_T1_n-\mu\Vert_1 + \Vert(\overline{\gamma}_T)^\top1_m-\nu\Vert_1.
\end{equation}
Moreover, after a final rounding step we have
\begin{equation}
    \Esp{}{f(\ROUND(\overline{\gamma}_T)) - f(\gamma^*)} \leq  \frac{9B_\sigma}{8}\sqrt{\frac{\radius}{T}}(2+\log(T)).
\end{equation}
%\end{thm}



==> sections/theorems/thm_stoch_smooth.tex <==
%\begin{thm}\label{thm:stochsmooth}
We assume that $f$ verifies 
\begin{equation}
    \langle\nabla f(\gamma) - \nabla f(\gamma^*),\gamma - \gamma^*\rangle\leq LD_{\KL} (\gamma^*, \gamma)
\end{equation}
which is true if $f$ is $L-$smooth for the norm $\Vert\cdot\Vert_1$.
let $0\leq\alpha\leq 1$, let the stepsize be $\eta_t = \frac{1}{Lt^\alpha}$ in the algorithm \ref{alg:stoch}, then the output $\overline{\gamma}_T$ after $T$ steps verifies
\begin{equation}
    \Esp{}{f(\overline{\gamma}_T)-f(\gamma^*)} \leq \frac{L\radius}{T^{1-\alpha}}.
\end{equation}
and the constraints are close to be verified:
\begin{equation}
    \Esp{}{c(\overline{\gamma}_T)}\leq  \frac{2(1-\alpha)\radius}{T^{\alpha}} + \frac{\radius}{T}.
\end{equation}
With a general choice of decreasing step-size we have 
\begin{equation}
    \Esp{}{f(\overline{\gamma}_T)-f(\gamma^*)} \leq \frac{\radius}{T\eta_T}.
\end{equation}
and
\begin{equation}
    \Esp{}{c(\overline{\gamma}_T)}\leq  \frac{2(1-\alpha)L\radius}{T}\sum_{t=1}^T\eta_t + \frac{\radius}{T}.
\end{equation}
%\end{thm}

==> sections/theorems/thm_var.tex <==
%\begin{thm}\label{thm:var}
If $f$ is $B$-Lipschitz for the norm $\Vert\cdot\Vert_1$, let $\radius = \Vert \log \mu\Vert_\infty + \Vert \log \nu\Vert_\infty$ and let the stepsize be $\eta_t = \frac{1}{B}\sqrt{\frac{4\radius}{5t}}$ in the algorithm \ref{alg:main}, then the output $\overline{\gamma}_T$ after $T$ steps verifies
\begin{equation}
    f(\overline{\gamma}_T) - f(\gamma^*) \leq  2B\sqrt{\frac{\radius}{5T}}(2+\log(T)),
\end{equation}
and the constraints are close to be verified
\begin{equation}
    c(\overline{\gamma}_T) \leq  9\sqrt{\frac{\radius}{5T}}(1+\log(T)),
\end{equation}
with

%\end{thm}
